Playing Psychic: Using Thought Trees to Predict Reasoning Models Accuracy on Coding Tasks

Recent advances in large language models (LLMs) have shown that test-time scaling can substantially improve model performance on complex tasks, particularly in the coding domain. Under this paradigm, models use a larger token budget during inference to generate intermediate reasoning traces before producing a final answer. However, current evaluations primarily rely on competitive programming benchmarks, which may not capture the full range of reasoning abilities. In this work, we perform a systematic study of frontier reasoning models to understand their performance on real-world coding benchmarks. To gain more insights into the performance of such models, we devise a programmatic way to {\em automatically generate} coding tasks of arbitrary difficulty and structure from existing benchmarks. Using this framework, our analysis reveals that the structure of a reasoning trace, not just its contents, is a strong predictor of correctness. Motivated by this, we propose structured thought-trees as means to represent reasoning traces. To illustrate their use, we train a lightweight classifier on features extracted from thought-trees to predict trace correctness, and demonstrate that flagging and retrying structurally anomalous traces based on the extracted features yields consistent gains at lower complexity levels.

==> figures/length_ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/feature_random_sample_all.pdf}
    \caption{\textbf{Impact of reasoning trace feature density on the predictive accuracy of random forest classifiers.} The plots illustrate the relationship between the number of randomly selected features and the model's ability to predict output correctness across CRUXEval, SAFIM, and CodeLingua for DeepSeek-R1 and QwQ models. Shaded regions represent the variance across simulation runs.}
    \label{fig:placeholder}
\end{figure}
